Numerical Approximation Methods for Antenna Radiation Patterns for Motus Wildlife Tracking Systems

As plans for offshore wind energy development increase in the US, the developing methods to monitor migratory birds and bats offshore is an important area of research. To contribute to this research, current guidance recommends the deployment of Motus Wildlife Tracking stations by each developer for pre- and post- construction monitoring. To understand the characteristics of each of the stations, calibration techniques are recommended for each deployment. Despite this, previous attempts to calibrate these stations has failed to provide sufficient detail to allow for high-resolution tracking techniques. In this paper, we introduce an affordable and robust methodology to calibrate stations in the off-shore environment and develop processes to turn this raw calibration data into a numerical approximation of the antennas radiation pattern.

==> extra_text.tex <==
\begin{comment}
Due to the nature of our calibration surveys, our calibration space was insufficiently filled and thus our k-means algorithm fails in the vertical plane (see Figure \ref{fig:Altitude_Information}). To approximate our radiation pattern, we flatten our data to two-dimensions and assume spherical symmetry. Future approaches to calibration as outlined in Section \ref{sec:future_work} will aim to remedy this assumption. \\\\
Knowing the structure of a general yagi antenna, we are able to discern this structure from our K-means data by seeing the largest 
\end{comment}
